To Wake-up or Not to Wake-up: Reducing Keyword False Alarm by Successive Refinement

Keyword spotting systems continuously process audio streams to detect keywords. One of the most challenging tasks in designing such systems is to reduce False Alarm (FA) which happens when the system falsely registers a keyword despite the keyword not being uttered. In this paper, we propose a simple yet elegant solution to this problem that follows from the law of total probability. We show that existing deep keyword spotting mechanisms can be improved by Successive Refinement, where the system first classifies whether the input audio is speech or not, followed by whether the input is keyword-like or not, and finally classifies which keyword was uttered. We show across multiple models with size ranging from 13K parameters to 2.41M parameters, the successive refinement technique reduces FA by up to a factor of 8 on in-domain held-out FA data, and up to a factor of 7 on out-of-domain (OOD) FA data. Further, our proposed approach is "plug-and-play" and can be applied to any deep keyword spotting model.

==> placeholders.tex <==
\begin{figure}[!th]
\begin{center}
\begin{minipage}[b]{\linewidth}
\centerline{\includegraphics[width=0.9\linewidth]{Figures/proposed_syst.pdf}}
\end{minipage}
\vspace{-0.5cm}
\caption{The proposed DCUnet-intraMVDR multichannel SE system.}
\vspace{-0.5cm}
\label{fig: proposed syst}
\end{center}
\end{figure}

\begin{table}[!th]
\vspace{-0.5cm}
\caption{Comparison of DCUnet-based multichannel SE schemes. }
\label{table: comp of dcunet based schemes}
\begin{center}
\begin{footnotesize}
%\begin{sc}
\setlength{\tabcolsep}{2pt} % let TeX compute the intercolumn space
\begin{tabular}{lcccc}
\toprule
 Methods & \# Params & PESQ & STOI & SNR \\
\midrule
 Mask-based MVDR & 1.27M & 2.00 & 0.966 & 16.67 \\
 Direct FS & 1.27M & 2.39 & 0.962 & 17.76 \\
 FS w/ intraMVDR (no comb. out) & 1.30M & 2.45 & 0.964 & 17.88 \\
 FS w/ intraMVDR & 1.30M & \textbf{2.55} & \textbf{0.970} & \textbf{18.93} \\
\bottomrule
\end{tabular}
%\end{sc}
\end{footnotesize}
\end{center}
\vspace{-0.5cm}
\end{table}

\begin{table}[!th]
\vspace{-0.5cm}
\caption{SE performance of the proposed DCUnet-intraMVDR system with different settings of intraMVDR levels.}
\vspace{-0.25cm}
\label{table: se performance for diff mvdr levels}
\begin{center}
\begin{footnotesize}
%\begin{sc}
\setlength{\tabcolsep}{2pt} % let TeX compute the intercolumn space
\begin{tabular}{llcccc}
\toprule
 Methods & & \# Params & PESQ & STOI & SNR \\
\midrule
\multirow{4}{*}{FS w/ intraMVDR} & Level 1 & 1.30M & 2.55 & 0.970 & 18.93 \\
 & Levels 1,2 & 1.38M & 2.57 & 0.973 & 20.43 \\
 & Levels 1,2,3 & 1.47M & 2.60 & \textbf{0.974} & \textbf{20.80} \\
 & Levels 1,2,3,4 & 1.56M & \textbf{2.64} & \textbf{0.974} & 20.63 \\
\midrule
 Mask-based MVDR & (Larger) & 1.62M & 2.01 & 0.966 & 16.81 \\
 Direct FS \, (Larger) &  & 1.62M & 2.44 & 0.965 & 18.31 \\
\bottomrule
\end{tabular}
%\end{sc}
\end{footnotesize}
\end{center}
\vspace{-0.5cm}
\end{table}

\begin{table}[!th]
\vspace{-0.5cm}
\caption{Comparison with SOTA methods on the CHiME-3 dataset.}
\vspace{-0.25cm}
\label{table: sota comp chime}
\begin{center}
\begin{footnotesize}
%\begin{sc}
\setlength{\tabcolsep}{3pt} % let TeX compute the intercolumn space
\begin{tabular}{lcccc}
\toprule 
 Methods & \# Params & PESQ & STOI & SNR \\
\midrule
 Noisy & - & 1.27 & 0.870 & 6.50 \\
 Neural BF \cite{erdogan2016improved} & - & 2.29 & - & 15.12 \\
 MVDR$\displaystyle _{GC}$ \cite{bu2019novel} & 0.5M & - & 0.952 & - \\
 rSDFCN \cite{liu2020multichannel} & 2.1M & 2.15 & 0.937 & -\\
 CA Dense U-Net \cite{tolooshams2020channel} & $>$20M & 2.44 & - & 18.64 \\
 %IC Conv-TasNet & 1.67M & 2.67 & 0.973 \\
 DCUnet-intraMVDR (ours) & 1.56M & \textbf{2.64} & \textbf{0.974} & \textbf{20.63} \\
 \bottomrule
\end{tabular}
%\end{sc}
\end{footnotesize}
\end{center}
\vspace{-0.5cm}
\end{table}


\begin{figure*}[!th]
\centering
\begin{minipage}[b]{0.24\linewidth}
\includegraphics[width=1.1\linewidth]{./Figures/irms_level1.eps}
\end{minipage}
%\hfill
\begin{minipage}[b]{0.24\linewidth}
\includegraphics[width=1.1\linewidth]{./Figures/irms_level2.eps}
\end{minipage}
%\hfill
\begin{minipage}[b]{0.24\linewidth}
\includegraphics[width=1.1\linewidth]{./Figures/irms_level3.eps}
\end{minipage}
%\hfill
\begin{minipage}[b]{0.24\linewidth}
\includegraphics[width=1.1\linewidth]{./Figures/irms_level4.eps}
\end{minipage}
\vspace{-0.2cm}
\caption{Visualizing the estimated speech and noise T-F masks in different levels of the intraMVDR block.}
\vspace{-0.2cm}
\label{fig: irms}
\end{figure*}


\begin{figure}[!th]
\centering
\begin{minipage}[b]{0.49\linewidth}
\includegraphics[width=1.1\linewidth]{./Figures/irms_level1.eps}
\end{minipage}
\hfill
\begin{minipage}[b]{0.49\linewidth}
\includegraphics[width=1.1\linewidth]{./Figures/irms_level2.eps}
\end{minipage}
\hfill
\begin{minipage}[b]{0.49\linewidth}
\includegraphics[width=1.1\linewidth]{./Figures/irms_level3.eps}
\end{minipage}
\hfill
\begin{minipage}[b]{0.49\linewidth}
\includegraphics[width=1.1\linewidth]{./Figures/irms_level4.eps}
\end{minipage}
\vspace{-0.2cm}
\caption{Visualizing the estimated speech and noise T-F masks in different levels of the intraMVDR block.}
\vspace{-0.2cm}
\label{fig: irms}
\end{figure}
